SketchyScene: Richly-Annotated Scene Sketches

We contribute the first large-scale dataset of scene sketches, SketchyScene, with the goal of advancing research on sketch understanding at both the object and scene level. The dataset is created through a novel and carefully designed crowdsourcing pipeline, enabling users to efficiently generate large quantities of realistic and diverse scene sketches. SketchyScene contains more than 29,000 scene-level sketches, 7,000+ pairs of scene templates and photos, and 11,000+ object sketches. All objects in the scene sketches have ground-truth semantic and instance masks. The dataset is also highly scalable and extensible, easily allowing augmenting and/or changing scene composition. We demonstrate the potential impact of SketchyScene by training new computational models for semantic segmentation of scene sketches and showing how the new dataset enables several applications including image retrieval, sketch colorization, editing, and captioning, etc. The dataset and code can be found at https://github.com/SketchyScene/SketchyScene.

==> macros.tex <==
\renewcommand{\textrightarrow}{$\rightarrow$}

%% the following commands are plagiarized from Ravi
\newcommand{\pcline }{\rule{0in}{0.0in}    }  % Spacing for pseudo-code.
\newcommand{\pctab  }{\hspace{0.10in}      }  % Pseudo-code indentation.
\newcommand{\pcbigtab  }{\hspace{1.75in}    }  % Pseudo-code indentation.
\newcommand{\pcasgn }{\mbox{$\leftarrow$}  }  % Pseudo-code assignment operator
%%\newcommand{\pcgreater}{\mbox{$\leftarrow$} } % Pseudo-code bigger operator
\newcommand{\pcomment}[1]{\mbox{// {\it #1}}}  % Pseudo-code comments.
\newcommand{\pckeyword}[1]{\mbox{{\bf #1}}}  % Pseudo-code keywords.
\newcommand{\pcspace}{\hspace{0.10in}}

\newcommand{\pcode}[1]{
    \footnotesize
    \vspace{-0.1in}
    \begin{minipage}{100in} % The width argument will be ignored:
                            % See lamport p. 99
    \begin{tabbing} \hspace{0.10in} \= \pctab \= \pctab \= \pctab \= \pctab \= \pctab \= \pctab \= \pctab \= \pctab \= \\
        #1
    \end{tabbing}
    \end{minipage}
%    \vspace{0.15in}
    }
%% enf of the pseudo code environment

\newcommand{\parallelkeyword}{\pckeyword{{\color{blue}parallel}}}

%%\newcommand{\Caption}[1]{\caption{\small {\em #1}}}
%%\newcommand{\Caption}[1]{\caption{{\em #1}}}
\newcommand{\Caption}[2]{\caption[#1]{{\footnotesize #1} {\footnotesize #2}}}
%%\newcommand{\Caption}[1]{\caption{\it \small {#1}}}

\newcommand{\tabtextsize}{\footnotesize}
\newcommand{\figtext}[1]{{\footnotesize #1}}

\newcommand{\invisible}[1]{{\color{white} #1}}
\newcommand{\emacsquote}[1]{{``#1''}}

\newcommand{\warning}[1]{{\it\color{red} #1}}
\newcommand{\note}[1]{{\it\color{blue} #1}}
\newcommand{\nothing}[1]{}
\newcommand{\psdraftboxDefault}{\psnodraftbox}

\definecolor{HaibinColor}{rgb}{1.0,0.65,0} % color for Haibin
\newcommand{\haibin}[1]{{\color{HaibinColor} Haibin: #1}}

\definecolor{KaloColor}{rgb}{1.0,0,0} % color for Kalo
\newcommand{\kalo}[1]{{\color{KaloColor}#1}}

\definecolor{CQColor}{rgb}{0.0,1.0,0.0} % color for Aaron
\newcommand{\cq}[1]{{\color{CQColor} CQ: #1}}

\definecolor{RZColor}{rgb}{0,0,1.0} % color for Richard
\newcommand{\rz}[1]{{\color{RZColor}#1}}

\definecolor{MPColor}{rgb}{0.8,0,0.2} % color for Marie-Paule
\newcommand{\MPaule}[1]{{\color{MPColor} #1}}
\newcommand{\MPComment}[1]{{\color{MPColor}  (Marie-Paule: #1)}}

\definecolor{ZhaoliangColor}{rgb}{1.0,0.0,1.0} % color for Zhaoliang
\newcommand{\zhaoliang}[1]{{\color{ZhaoliangColor} Zhaoliang: #1}}

%\newcommand{\rev}[1]{{\color{red}#1}}
\newcommand{\rev}[1]{#1}


%% Symbols
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bm}{\mathbf{m}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}


%{ReviewerColor}{rgb}{0.3,0.3,1.0} % color for anti-sith
%\newcommand{\reviewer}[1]{{\color{ReviewerColor} Reviewer: #1}}

% \liyi{Use this to quickly tune options between paragraph or subsection for apps under application.tex}
\newcommand{\appsection}[1]{\paragraph{#1}}
%\renewcommand{\appsection}[1]{\paragraph{#1}}

\ifdefined\mainonly
\else
\newcommand{\mainonly}{0}
\fi

\linespread{0.99}

